Secure and Reliable Key Agreement with Physical Unclonable Functions

Different transforms used in binding a secret key to correlated physical-identifier outputs are compared. Decorrelation efficiency is the metric used to determine transforms that give highly-uncorrelated outputs. Scalar quantizers are applied to transform outputs to extract uniformly distributed bit sequences to which secret keys are bound. A set of transforms that perform well in terms of the decorrelation efficiency is applied to ring oscillator (RO) outputs to improve the uniqueness and reliability of extracted bit sequences, to reduce the hardware area and information leakage about the key and RO outputs, and to maximize the secret-key length. Low-complexity error-correction codes are proposed to illustrate two complete key-binding systems with perfect secrecy, and better secret-key and privacy-leakage rates than existing methods. A reference hardware implementation is also provided to demonstrate that the transform-coding approach occupies a small hardware area.

==> macro.tex <==
\tikzstyle{block} = [draw, fill=blue!5, rectangle, rounded corners,
    minimum height=2em, minimum width=6em]
\tikzstyle{input} = [draw, fill=green!5, rectangle, rounded corners,
    minimum height=2em, minimum width=4em]
\tikzstyle{chan} = [draw, fill=red!5, rectangle, rounded corners,
    minimum height=2em, minimum width=4em]
\tikzstyle{output} = [coordinate]
\tikzstyle{pinstyle} = [pin edge={to-,thin,black}]
\tikzstyle{block2} = [draw, rectangle,  minimum height=1.5em, minimum width=2em]
\tikzstyle{sum} = [draw, circle, inner sep=0pt, node distance=1cm]

\tikzstyle{block3} = [draw, rectangle,  minimum height=1.5cm, minimum width=1.5cm]
\tikzstyle{block4} = [ rectangle,  minimum height=1.5cm, minimum width=1.5cm]
\tikzstyle{block5} = [draw, rectangle,  minimum height=1.5em, minimum width=1.5cm]
\tikzstyle{block5b} = [ rectangle,  minimum height=1.5em, minimum width=2cm]


% Terminals
\newcommand{\tone}{\ensuremath{T_1}}
\newcommand{\ttwo}{\ensuremath{T_2}}
\newcommand{\tr}{\ensuremath{r}}

% W - messages
\newcommand{\w}{\ensuremath{W}}
\newcommand{\wone}{\ensuremath{W_1}}
\newcommand{\wtwo}{\ensuremath{W_2}}
\newcommand{\wonehat}{\ensuremath{\hat{W}_1}}
\newcommand{\wtwohat}{\ensuremath{\hat{W}_2}}

% x
\newcommand{\x}{\ensuremath{X}}
\newcommand{\xone}{\ensuremath{X_1}}
\newcommand{\xtwo}{\ensuremath{X_2}}
\newcommand{\xr}{\ensuremath{X_r}}

% y
\newcommand{\Y}{\ensuremath{Y}}
\newcommand{\yr}{\ensuremath{Y_r}}
\newcommand{\yone}{\ensuremath{Y_1}}
\newcommand{\ytwo}{\ensuremath{Y_2}}




% Z - noise
\newcommand{\zone}{\ensuremath{Z_1}}
\newcommand{\ztwo}{\ensuremath{Z_2}}
\newcommand{\zr}{\ensuremath{Z_r}}

% p
\newcommand{\Pone}{\ensuremath{P_1}}
\newcommand{\Ptwo}{\ensuremath{P_2}}
\newcommand{\Prel}{\ensuremath{P_r}}

% N
\newcommand{\Nr}{\ensuremath{N_r}}
\newcommand{\None}{\ensuremath{N_1}}
\newcommand{\Ntwo}{\ensuremath{N_2}}

 \newcommand{\mc}[1]{\mathcal{#1}}
\newcommand{\Absatz}[0]{\vspace*{5mm}}
\newcommand{\eq}[2]{\begin{equation} #1 \label{#2}\end{equation}}
\newcommand{\ve}[1]{\uline{\smash #1}}
\newcommand{\tn}[1]{\textnormal{#1}}
\newcommand{\truth}{\mbox{\textbb{1}}}
\newcommand{\hY}{\hat Y_r}
\newcommand{\hy}{\hat y_r}
\newcommand{\hyri}{\hat y_{ri}}
\newcommand{\nMAC}{n_{\text{MAC}}}
\newcommand{\nBC}{n_{\text{BC}}}
\newcommand{\yhcard}{\ensuremath{L}}
\newcommand{\ycard}{\ensuremath{|\mc Y_r |}}


\tikzstyle{block} = [draw, fill=blue!5, rectangle, rounded corners,
    minimum height=2em, minimum width=6em]
\tikzstyle{input} = [draw, fill=green!5, rectangle, rounded corners,
    minimum height=2em, minimum width=4em]
\tikzstyle{chan} = [draw, fill=red!5, rectangle, rounded corners,
    minimum height=2em, minimum width=4em]
\tikzstyle{output} = [coordinate]
\tikzstyle{pinstyle} = [pin edge={to-,thin,black}]
\tikzstyle{block2} = [draw, rectangle, 
    minimum height=1.5em, minimum width=2em]
\tikzstyle{sum} = [draw, circle, inner sep=0pt, node distance=1cm]


==> pgflibrarytikzcircuits.code.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% %
% pgflibrarytikzcircuits.code.tex %
% %
% Version 0.0.1 %
% %
% Authors: Juergen Werber and Christoph Bartoschek %
% Email: bartoschek -at- or.uni-bonn.de %
% %
% This file may be distributed and/or modified %
% 1. under the LaTeX Project Public License Version 1.3 or later %
% and/or %
% 2. under the GNU Public License Version 2 or later. %
% %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%% USAGE EXAMPLE %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \documentclass{article}
% \usepackage{tikz}
% \usetikzlibrary{circuits}
%
% \begin{document}
% \begin{tikzpicture}[scale=0.5,cktbaselength=0.5pt]
% \draw (6,0) node[nand2ni,anchor=tip,draw] (n4) {}
% (n4.z) -- +(0mm,-5mm)
% (n4.b) |- ++(10mm,2mm) -- ++(0mm,2mm)
% node[and2in,anchor=z,draw,fill=gray] (n3) {}
% (n4.a) |- ++(-10mm,2mm) -- ++(0mm,2mm)
% node[or3nni,anchor=tip,draw] (n2) {}
% (n3.b) -- +(0mm,5mm) node[above] {$i_5$}
% (n3.a) |- ++(-5mm,2mm)
% coordinate (p) -- +(0mm,5mm) node[above] {$i_4$}
% (n2.c) |- (p)
% (n2.b) |- ++(6mm,12mm) -- +(0mm,5mm) node[above] {$i_3$}
% (n2.a) -- +(0mm,8mm)
% node[and2,anchor=tip,draw] (n1) {}
% (n1.b) -- +(0mm,5mm) node[above] {$i_2$}
% (n1.a) -- +(0mm,5mm) node[above] {$i_1$};
% \end{tikzpicture}
% \end{document}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\pgfsetcktbaselength#1{\def\cktbaselength{#1}}
\pgfsetcktbaselength{2pt}
\tikzoption{cktbaselength}{\pgfsetcktbaselength{#1}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\cktsetbasexandyvec{%
\pgfsetxvec{\pgfpoint{\baselength}{0pt}}
\pgfsetyvec{\pgfpoint{0pt}{\baselength}}
}
\def\cktsetcktbasexandyvec{%
\pgfsetxvec{\pgfpoint{\cktbaselength}{0pt}}
\pgfsetyvec{\pgfpoint{0pt}{\cktbaselength}}
}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\cktdrawtrianglenonclosed{%
\pgfpathmoveto{\pgfpointorigin}
\pgfpathlineto{\pgfpointxy{10}{20}}
\pgfpathlineto{\pgfpointxy{-10}{20}}
}
\def\cktdrawfitwotrunk{%
\pgfpathmoveto{\pgfpointxy{20}{28}}
\pgfpathcurveto{\pgfpointxy{20}{4}}{\pgfpointxy{8}{0}}{\pgfpointorigin}
\pgfpathcurveto{\pgfpointxy{-8}{0}}{\pgfpointxy{-20}{4}}{\pgfpointxy{-20}{28}}
}
\def\cktdrawandtwoshape{%
\cktdrawfitwotrunk
\pgfpathclose
}
\def\cktdrawortwoshape{%
\cktdrawfitwotrunk
\pgfpathcurveto{\pgfpointxy{-6}{16}}{\pgfpointxy{6}{16}}{\pgfpointxy{20}{28}}
\pgfpathclose
}
\def\cktdrawfithreetrunk{%
\pgfpathmoveto{\pgfpointxy{30}{30}}
\pgfpathcurveto{\pgfpointxy{30}{6}}{\pgfpointxy{12}{0}}{\pgfpointorigin}
\pgfpathcurveto{\pgfpointxy{-12}{0}}{\pgfpointxy{-30}{6}}{\pgfpointxy{-30}{30}}
}
\def\cktdrawandthreeshape{%
\cktdrawfithreetrunk
\pgfpathclose
}
\def\cktdraworthreeshape{%
\cktdrawfithreetrunk
\pgfpathcurveto{\pgfpointxy{-10}{16}}{\pgfpointxy{10}{16}}{\pgfpointxy{30}{30}}
\pgfpathclose
}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\cktlocateortwoaanchor{%
\pgfpointcurveattime{0.2452}{\pgfpointxy{-20}{28}}{\pgfpointxy{-6}{16}}{\pgfpointxy{6}{16}}{\pgfpointxy{20}{28}}%
}
\def\cktlocateorthreeaanchor{%
\pgfpointcurveattime{0.1667}{\pgfpointxy{-30}{30}}{\pgfpointxy{-10}{16}}{\pgfpointxy{10}{16}}{\pgfpointxy{30}{30}}%
}
\def\cktlocateorthreebanchor{%
\pgfpointcurveattime{0.5}{\pgfpointxy{-30}{30}}{\pgfpointxy{-10}{16}}{\pgfpointxy{10}{16}}{\pgfpointxy{30}{30}}%
}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\cktdrawzinversion{%
\@tempdima=\baselength
\pgfpathcircle{\pgfpointxy{0}{-3}}{3\@tempdima}
}
\def\cktdrawandtwoainversion{%
\@tempdima=\baselength
\pgfpathcircle{\pgfpointxy{-10}{31}}{3\@tempdima}
}
\def\cktdrawandtwobinversion{%
\@tempdima=\baselength
\pgfpathcircle{\pgfpointxy{10}{31}}{3\@tempdima}
}
\def\cktdrawortwoainversion{%
\@tempdima=\baselength
\pgfpathcircle{\pgfpoint{-10\@tempdima}{\ycirccenter}}{3\@tempdima}
}
\def\cktdrawortwobinversion{%
\@tempdima=\baselength
\pgfpathcircle{\pgfpoint{10\@tempdima}{\ycirccenter}}{3\@tempdima}
}
\def\cktdrawandthreeainversion{%
\@tempdima=\baselength
\pgfpathcircle{\pgfpointxy{-20}{33}}{3\@tempdima}
}
\def\cktdrawandthreebinversion{%
\@tempdima=\baselength
\pgfpathcircle{\pgfpointxy{0}{33}}{3\@tempdima}
}
\def\cktdrawandthreecinversion{%
\@tempdima=\baselength
\pgfpathcircle{\pgfpointxy{20}{33}}{3\@tempdima}
}
\def\cktdraworthreeainversion{%
\@tempdima=\baselength
\pgfpathcircle{\pgfpoint{-20\@tempdima}{\ycirccenter}}{3\@tempdima}
}
\def\cktdraworthreebinversion{%
\pgfpointcurveattime{0.5}{\pgfpointxy{-30}{30}}{\pgfpointxy{-10}{16}}{\pgfpointxy{10}{16}}{\pgfpointxy{30}{30}}%
\@tempdima=\baselength
\advance\pgf@y by 3\@tempdima
\pgfpathcircle{\pgfpoint{\pgf@x}{\pgf@y}}{3\@tempdima}
}
\def\cktdraworthreecinversion{%
\@tempdima=\baselength
\pgfpathcircle{\pgfpoint{20\@tempdima}{\ycirccenter}}{3\@tempdima}
}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\pgfdeclareshape{buffer}{
\saveddimen{\baselength}{
\pgf@x=\cktbaselength
}
% TODO: chose barycenter for center instead?
\anchor{center}{ \cktsetbasexandyvec \pgfpointxy{0}{10} }
\anchor{north west}{ \cktsetbasexandyvec \pgfpointxy{-10}{20} }
\anchor{north}{ \cktsetbasexandyvec \pgfpointxy{0}{20} }
\anchor{north east}{ \cktsetbasexandyvec \pgfpointxy{10}{20} }
\anchor{west}{ \cktsetbasexandyvec \pgfpointxy{-10}{10} }
\anchor{east}{ \cktsetbasexandyvec \pgfpointxy{10}{10} }
\anchor{south west}{ \cktsetbasexandyvec \pgfpointxy{-10}{0} }
\anchor{south}{ \pgfpointorigin }
\anchor{south east}{ \cktsetbasexandyvec \pgfpointxy{10}{0} }
\anchor{a}{ \cktsetbasexandyvec \pgfpointxy{0}{20} }
\anchor{z}{ \pgfpointorigin }
\anchor{tip}{ \pgfpointorigin }
\backgroundpath{
\cktsetbasexandyvec
\cktdrawtrianglenonclosed
\pgfpathclose
}
}
\pgfdeclareshape{inverter}{
\inheritsavedanchors[from=buffer]
\inheritanchor[from=buffer]{center}
\inheritanchor[from=buffer]{north west}
\inheritanchor[from=buffer]{north}
\inheritanchor[from=buffer]{north east}
\inheritanchor[from=buffer]{tip}
\inheritanchor[from=buffer]{a}
\anchor{west}{ \cktsetbasexandyvec \pgfpointxy{-10}{7} }
\anchor{east}{ \cktsetbasexandyvec \pgfpointxy{10}{7} }
\anchor{south west}{ \cktsetbasexandyvec \pgfpointxy{-10}{-6} }
\anchor{south}{ \cktsetbasexandyvec \pgfpointxy{0}{-6} }
\anchor{south east}{ \cktsetbasexandyvec \pgfpointxy{10}{-6} }
\anchor{z}{ \cktsetbasexandyvec \pgfpointxy{0}{-6} }
\backgroundpath{
\cktsetbasexandyvec
% The inverter looks nicer if the path is not closed.
\cktdrawtrianglenonclosed
\pgfpathlineto{\pgfpointorigin}
\cktdrawzinversion
}
}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\pgfdeclareshape{and2}{
\saveddimen{\baselength}{
\pgf@x=\cktbaselength
}
% TODO: chose barycenter for center instead?
\anchor{center}{ \cktsetbasexandyvec \pgfpointxy{0}{14} }
\anchor{north west}{ \cktsetbasexandyvec \pgfpointxy{-20}{28} }
\anchor{north}{ \cktsetbasexandyvec \pgfpointxy{0}{28} }
\anchor{north east}{ \cktsetbasexandyvec \pgfpointxy{20}{28} }
\anchor{west}{ \cktsetbasexandyvec \pgfpointxy{-20}{14} }
\anchor{east}{ \cktsetbasexandyvec \pgfpointxy{20}{14} }
\anchor{south west}{ \cktsetbasexandyvec \pgfpointxy{-20}{0} }
\anchor{south}{ \pgfpointorigin }
\anchor{south east}{ \cktsetbasexandyvec \pgfpointxy{20}{0} }
\anchor{a}{ \cktsetbasexandyvec \pgfpointxy{-10}{28} }
\anchor{b}{ \cktsetbasexandyvec \pgfpointxy{10}{28} }
\anchor{z}{ \pgfpointorigin }
\anchor{tip}{ \pgfpointorigin }
\backgroundpath{
\cktsetbasexandyvec
\cktdrawandtwoshape
}
}
\pgfdeclareshape{nand2ii}{
\inheritsavedanchors[from=and2]
\inheritanchor[from=and2]{center}
\inheritanchor[from=and2]{west}
\inheritanchor[from=and2]{east}
\inheritanchor[from=and2]{tip}
\anchor{north west}{ \cktsetbasexandyvec \pgfpointxy{-20}{34} }
\anchor{north}{ \cktsetbasexandyvec \pgfpointxy{0}{34} }
\anchor{north east}{ \cktsetbasexandyvec \pgfpointxy{20}{34} }
\anchor{south west}{ \cktsetbasexandyvec \pgfpointxy{-20}{-6} }
\anchor{south}{ \cktsetbasexandyvec \pgfpointxy{0}{-6} }
\anchor{south east}{ \cktsetbasexandyvec \pgfpointxy{20}{-6} }
\anchor{a}{ \cktsetbasexandyvec \pgfpointxy{-10}{34} }
\anchor{b}{ \cktsetbasexandyvec \pgfpointxy{10}{34} }
\anchor{z}{ \cktsetbasexandyvec \pgfpointxy{0}{-6} }
\backgroundpath{
\cktsetbasexandyvec
\cktdrawandtwoshape
\cktdrawandtwoainversion
\cktdrawandtwobinversion
\cktdrawzinversion
}
}
\pgfdeclareshape{and2in}{
\inheritsavedanchors[from=and2]
\inheritanchor[from=and2]{center}
\inheritanchor[from=nand2ii]{north west}
\inheritanchor[from=nand2ii]{north}
\inheritanchor[from=nand2ii]{north east}
\inheritanchor[from=and2]{south east}
\inheritanchor[from=and2]{south}
\inheritanchor[from=and2]{south west}
\inheritanchor[from=nand2ii]{a}
\inheritanchor[from=and2]{b}
\inheritanchor[from=and2]{z}
\inheritanchor[from=and2]{tip}
\anchor{west}{ \cktsetbasexandyvec \pgfpointxy{-20}{17} }
\anchor{east}{ \cktsetbasexandyvec \pgfpointxy{20}{17} }
\backgroundpath{
\cktsetbasexandyvec
\cktdrawandtwoshape
\cktdrawandtwoainversion
}
}
\pgfdeclareshape{and2ni}{
\inheritsavedanchors[from=and2]
\inheritanchor[from=and2]{center}
\inheritanchor[from=nand2ii]{north west}
\inheritanchor[from=nand2ii]{north}
\inheritanchor[from=nand2ii]{north east}
\inheritanchor[from=and2in]{west}
\inheritanchor[from=and2in]{east}
\inheritanchor[from=and2]{south east}
\inheritanchor[from=and2]{south}
\inheritanchor[from=and2]{south west}
\inheritanchor[from=and2]{a}
\inheritanchor[from=nand2ii]{b}
\inheritanchor[from=and2]{z}
\inheritanchor[from=and2]{tip}
\backgroundpath{
\cktsetbasexandyvec
\cktdrawandtwoshape
\cktdrawandtwobinversion
}
}
\pgfdeclareshape{and2ii}{
\inheritsavedanchors[from=and2]
\inheritanchor[from=and2]{center}
\inheritanchor[from=nand2ii]{north west}
\inheritanchor[from=nand2ii]{north}
\inheritanchor[from=nand2ii]{north east}
\inheritanchor[from=and2in]{west}
\inheritanchor[from=and2in]{east}
\inheritanchor[from=and2]{south east}
\inheritanchor[from=and2]{south}
\inheritanchor[from=and2]{south west}
\inheritanchor[from=nand2ii]{a}
\inheritanchor[from=nand2ii]{b}
\inheritanchor[from=and2]{z}
\inheritanchor[from=and2]{tip}
\backgroundpath{
\cktsetbasexandyvec
\cktdrawandtwoshape
\cktdrawandtwoainversion
\cktdrawandtwobinversion
}
}
\pgfdeclareshape{nand2}{
\inheritsavedanchors[from=and2]
\inheritanchor[from=and2]{center}
\inheritanchor[from=and2]{north west}
\inheritanchor[from=and2]{north}
\inheritanchor[from=and2]{north east}
\inheritanchor[from=nand2ii]{south east}
\inheritanchor[from=nand2ii]{south}
\inheritanchor[from=nand2ii]{south west}
\inheritanchor[from=and2]{a}
\inheritanchor[from=and2]{b}
\inheritanchor[from=nand2ii]{z}
\inheritanchor[from=and2]{tip}
\anchor{west}{ \cktsetbasexandyvec \pgfpointxy{-20}{11} }
\anchor{east}{ \cktsetbasexandyvec \pgfpointxy{20}{11} }
\backgroundpath{
\cktsetbasexandyvec
\cktdrawandtwoshape
\cktdrawzinversion
}
}
\pgfdeclareshape{nand2in}{
\inheritsavedanchors[from=and2]
\inheritanchor[from=and2]{center}
\inheritanchor[from=nand2ii]{north west}
\inheritanchor[from=nand2ii]{north}
\inheritanchor[from=nand2ii]{north east}
\inheritanchor[from=nand2ii]{west}
\inheritanchor[from=nand2ii]{east}
\inheritanchor[from=nand2ii]{south east}
\inheritanchor[from=nand2ii]{south}
\inheritanchor[from=nand2ii]{south west}
\inheritanchor[from=nand2ii]{a}
\inheritanchor[from=and2]{b}
\inheritanchor[from=nand2ii]{z}
\inheritanchor[from=and2]{tip}
\backgroundpath{
\cktsetbasexandyvec
\cktdrawandtwoshape
\cktdrawandtwoainversion
\cktdrawzinversion
}
}
\pgfdeclareshape{nand2ni}{
\inheritsavedanchors[from=and2]
\inheritanchor[from=and2]{center}
\inheritanchor[from=nand2ii]{north west}
\inheritanchor[from=nand2ii]{north}
\inheritanchor[from=nand2ii]{north east}
\inheritanchor[from=nand2ii]{west}
\inheritanchor[from=nand2ii]{east}
\inheritanchor[from=nand2ii]{south east}
\inheritanchor[from=nand2ii]{south}
\inheritanchor[from=nand2ii]{south west}
\inheritanchor[from=and2]{a}
\inheritanchor[from=nand2ii]{b}
\inheritanchor[from=nand2ii]{z}
\inheritanchor[from=and2]{tip}
\backgroundpath{
\cktsetbasexandyvec
\cktdrawandtwoshape
\cktdrawandtwobinversion
\cktdrawzinversion
}
}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\pgfdeclareshape{or2}{
\inheritsavedanchors[from=and2]
\inheritanchor[from=and2]{center}
\inheritanchor[from=and2]{north west}
\inheritanchor[from=and2]{north}
\inheritanchor[from=and2]{north east}
\inheritanchor[from=and2]{west}
\inheritanchor[from=and2]{east}
\inheritanchor[from=and2]{south east}
\inheritanchor[from=and2]{south}
\inheritanchor[from=and2]{south west}
\inheritanchor[from=and2]{tip}
\inheritanchor[from=and2]{z}
\anchor{a}{ \cktsetbasexandyvec \cktlocateortwoaanchor }
\anchor{b}{ \cktsetbasexandyvec \cktlocateortwoaanchor \pgf@x=-\pgf@x }
\backgroundpath{
\cktsetbasexandyvec
\cktdrawortwoshape
}
}
\pgfdeclareshape{nor2ii}{
\inheritsavedanchors[from=and2]
\saveddimen\ycirccenter{
\cktsetcktbasexandyvec
\pgfpointxy{24.685}{0}
}
\inheritanchor[from=and2]{center}
\inheritanchor[from=nand2]{west} % TODO: This is not exact
\inheritanchor[from=nand2]{east} % TODO: This is not exact
\inheritanchor[from=nand2ii]{south east}
\inheritanchor[from=nand2ii]{south}
\inheritanchor[from=nand2ii]{south west}
\inheritanchor[from=and2]{tip}
\inheritanchor[from=nand2ii]{z}
\anchor{north west}{ \cktsetbasexandyvec \pgfpointxy{-20}{3} \advance\pgf@y by \ycirccenter }
\anchor{north}{ \cktsetbasexandyvec \pgfpointxy{0}{3} \advance\pgf@y by \ycirccenter }
\anchor{north east}{ \cktsetbasexandyvec \pgfpointxy{20}{3} \advance\pgf@y by \ycirccenter }
\anchor{a}{ \cktsetbasexandyvec \pgfpointxy{-10}{3} \advance\pgf@y by \ycirccenter }
\anchor{b}{ \cktsetbasexandyvec \pgfpointxy{10}{3} \advance\pgf@y by \ycirccenter }
\backgroundpath{
\cktsetbasexandyvec
\cktdrawortwoshape
\cktdrawortwoainversion
\cktdrawortwobinversion
\cktdrawzinversion
}
}
\pgfdeclareshape{or2in}{
\inheritsavedanchors[from=nor2ii]
\inheritanchor[from=and2]{center}
\inheritanchor[from=nor2ii]{north west}
\inheritanchor[from=nor2ii]{north}
\inheritanchor[from=nor2ii]{north east}
\inheritanchor[from=nand2ii]{east} % TODO: This is not exact
\inheritanchor[from=nand2ii]{west} % TODO: This is not exact
\inheritanchor[from=and2]{south east}
\inheritanchor[from=and2]{south}
\inheritanchor[from=and2]{south west}
\inheritanchor[from=and2]{tip}
\inheritanchor[from=nor2ii]{a}
\inheritanchor[from=or2]{b}
\inheritanchor[from=and2]{z}
\backgroundpath{
\cktsetbasexandyvec
\cktdrawortwoshape
\cktdrawortwoainversion
}
}
\pgfdeclareshape{or2ni}{
\inheritsavedanchors[from=nor2ii]
\inheritanchor[from=and2]{center}
\inheritanchor[from=nor2ii]{north west}
\inheritanchor[from=nor2ii]{north}
\inheritanchor[from=nor2ii]{north east}
\inheritanchor[from=or2in]{west}
\inheritanchor[from=or2in]{east}
\inheritanchor[from=and2]{south east}
\inheritanchor[from=and2]{south}
\inheritanchor[from=and2]{south west}
\inheritanchor[from=and2]{tip}
\inheritanchor[from=or2]{a}
\inheritanchor[from=nor2ii]{b}
\inheritanchor[from=and2]{z}
\backgroundpath{
\cktsetbasexandyvec
\cktdrawortwoshape
\cktdrawortwobinversion
}
}
\pgfdeclareshape{or2ii}{
\inheritsavedanchors[from=nor2ii]
\inheritanchor[from=and2]{center}
\inheritanchor[from=nor2ii]{north west}
\inheritanchor[from=nor2ii]{north}
\inheritanchor[from=nor2ii]{north east}
\inheritanchor[from=or2in]{west}
\inheritanchor[from=or2in]{east}
\inheritanchor[from=and2]{south east}
\inheritanchor[from=and2]{south}
\inheritanchor[from=and2]{south west}
\inheritanchor[from=and2]{tip}
\inheritanchor[from=nor2ii]{a}
\inheritanchor[from=nor2ii]{b}
\inheritanchor[from=and2]{z}
\backgroundpath{
\cktsetbasexandyvec
\cktdrawortwoshape
\cktdrawortwoainversion
\cktdrawortwobinversion
}
}
\pgfdeclareshape{nor2}{
\inheritsavedanchors[from=and2]
\inheritanchor[from=and2]{center}
\inheritanchor[from=and2]{north west}
\inheritanchor[from=and2]{north}
\inheritanchor[from=and2]{north east}
\inheritanchor[from=nand2]{east}
\inheritanchor[from=nand2]{west}
\inheritanchor[from=nand2ii]{south east}
\inheritanchor[from=nand2ii]{south}
\inheritanchor[from=nand2ii]{south west}
\inheritanchor[from=and2]{tip}
\inheritanchor[from=or2]{a}
\inheritanchor[from=or2]{b}
\inheritanchor[from=nor2ii]{z}
\backgroundpath{
\cktsetbasexandyvec
\cktdrawortwoshape
\cktdrawzinversion
}
}
\pgfdeclareshape{nor2in}{
\inheritsavedanchors[from=nor2ii]
\inheritanchor[from=and2]{center}
\inheritanchor[from=nor2ii]{north west}
\inheritanchor[from=nor2ii]{north}
\inheritanchor[from=nor2ii]{north east}
\inheritanchor[from=nor2ii]{west}
\inheritanchor[from=nor2ii]{east}
\inheritanchor[from=nand2ii]{south east}
\inheritanchor[from=nand2ii]{south}
\inheritanchor[from=nand2ii]{south west}
\inheritanchor[from=and2]{tip}
\inheritanchor[from=nor2ii]{a}
\inheritanchor[from=or2]{b}
\inheritanchor[from=nor2ii]{z}
\backgroundpath{
\cktsetbasexandyvec
\cktdrawortwoshape
\cktdrawortwoainversion
\cktdrawzinversion
}
}
\pgfdeclareshape{nor2ni}{
\inheritsavedanchors[from=nor2ii]
\inheritanchor[from=and2]{center}
\inheritanchor[from=nor2ii]{north west}
\inheritanchor[from=nor2ii]{north}
\inheritanchor[from=nor2ii]{north east}
\inheritanchor[from=nor2ii]{west}
\inheritanchor[from=nor2ii]{east}
\inheritanchor[from=nand2ii]{south east}
\inheritanchor[from=nand2ii]{south}
\inheritanchor[from=nand2ii]{south west}
\inheritanchor[from=and2]{tip}
\inheritanchor[from=or2]{a}
\inheritanchor[from=nor2ii]{b}
\inheritanchor[from=nor2ii]{z}
\backgroundpath{
\cktsetbasexandyvec
\cktdrawortwoshape
\cktdrawortwobinversion
\cktdrawzinversion
}
}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\pgfdeclareshape{and3}{
\inheritsavedanchors[from=and2]
\inheritanchor[from=and2]{center}
\inheritanchor[from=and2]{tip}
\inheritanchor[from=and2]{z}
\anchor{north west}{ \cktsetbasexandyvec \pgfpointxy{-30}{30} }
\anchor{north}{ \cktsetbasexandyvec \pgfpointxy{0}{30} }
\anchor{north east}{ \cktsetbasexandyvec \pgfpointxy{30}{30} }
\anchor{west}{ \cktsetbasexandyvec \pgfpointxy{-30}{15} }
\anchor{east}{ \cktsetbasexandyvec \pgfpointxy{30}{15} }
\anchor{south west}{ \cktsetbasexandyvec \pgfpointxy{-30}{0} }
\anchor{south}{ \pgfpointorigin }
\anchor{south east}{ \cktsetbasexandyvec \pgfpointxy{30}{0} }
\anchor{a}{ \cktsetbasexandyvec \pgfpointxy{-20}{30} }
\anchor{b}{ \cktsetbasexandyvec \pgfpointxy{0}{30} }
\anchor{c}{ \cktsetbasexandyvec \pgfpointxy{20}{30} }
\backgroundpath{
\cktsetbasexandyvec
\cktdrawandthreeshape
}
}
\pgfdeclareshape{nand3iii}{
\inheritsavedanchors[from=and2]
\inheritanchor[from=and2]{center}
\inheritanchor[from=and2]{tip}
\inheritanchor[from=nand2ii]{z}
\inheritanchor[from=and3]{west}
\inheritanchor[from=and3]{east}
\anchor{north west}{ \cktsetbasexandyvec \pgfpointxy{-30}{36} }
\anchor{north}{ \cktsetbasexandyvec \pgfpointxy{0}{36} }
\anchor{north east}{ \cktsetbasexandyvec \pgfpointxy{30}{36} }
\anchor{south west}{ \cktsetbasexandyvec \pgfpointxy{-30}{-6} }
\anchor{south}{ \cktsetbasexandyvec \pgfpointxy{0}{-6} }
\anchor{south east}{ \cktsetbasexandyvec \pgfpointxy{30}{-6} }
\anchor{a}{ \cktsetbasexandyvec \pgfpointxy{-20}{36} }
\anchor{b}{ \cktsetbasexandyvec \pgfpointxy{0}{36} }
\anchor{c}{ \cktsetbasexandyvec \pgfpointxy{20}{36} }
\backgroundpath{
\cktsetbasexandyvec
\cktdrawandthreeshape
\cktdrawandthreeainversion
\cktdrawandthreebinversion
\cktdrawandthreecinversion
\cktdrawzinversion
}
}
\pgfdeclareshape{and3nni}{
\inheritsavedanchors[from=and2]
\inheritanchor[from=and2]{center}
\inheritanchor[from=and2]{tip}
\inheritanchor[from=and2]{z}
\inheritanchor[from=nand3iii]{north west}
\inheritanchor[from=nand3iii]{north}
\inheritanchor[from=nand3iii]{north east}
\inheritanchor[from=and3]{south west}
\inheritanchor[from=and3]{south}
\inheritanchor[from=and3]{south east}
\inheritanchor[from=and3]{a}
\inheritanchor[from=and3]{b}
\inheritanchor[from=nand3iii]{c}
\anchor{west}{ \cktsetbasexandyvec \pgfpointxy{-30}{18} }
\anchor{east}{ \cktsetbasexandyvec \pgfpointxy{30}{18} }
\backgroundpath{
\cktsetbasexandyvec
\cktdrawandthreeshape
\cktdrawandthreecinversion
}
}
\pgfdeclareshape{or3}{
\inheritsavedanchors[from=and2]
\inheritanchor[from=and2]{center}
\inheritanchor[from=and2]{tip}
\inheritanchor[from=and2]{z}
\anchor{north west}{ \cktsetbasexandyvec \pgfpointxy{-30}{30} }
\anchor{north}{ \cktsetbasexandyvec \pgfpointxy{0}{30} }
\anchor{north east}{ \cktsetbasexandyvec \pgfpointxy{30}{30} }
\anchor{west}{ \cktsetbasexandyvec \pgfpointxy{-30}{15} }
\anchor{east}{ \cktsetbasexandyvec \pgfpointxy{30}{15} }
\anchor{south west}{ \cktsetbasexandyvec \pgfpointxy{-30}{0} }
\anchor{south}{ \pgfpointorigin }
\anchor{south east}{ \cktsetbasexandyvec \pgfpointxy{30}{0} }
\anchor{a}{ \cktsetbasexandyvec \cktlocateorthreeaanchor }
\anchor{b}{ \cktsetbasexandyvec \cktlocateorthreebanchor }
\anchor{c}{ \cktsetbasexandyvec \cktlocateorthreeaanchor \pgf@x=-\pgf@x }
\backgroundpath{
\cktsetbasexandyvec
\cktdraworthreeshape
}
}
\pgfdeclareshape{nor3iii}{
\inheritsavedanchors[from=and2]
\inheritanchor[from=and2]{center}
\inheritanchor[from=and2]{tip}
\inheritanchor[from=nand2ii]{z}
\saveddimen\ycirccenter{
\cktsetcktbasexandyvec
\pgfpointxy{27.505}{0}
}
\anchor{north west}{ \cktsetbasexandyvec \pgfpointxy{-30}{30.505} }
\anchor{north}{ \cktsetbasexandyvec \pgfpointxy{0}{30.505} }
\anchor{north east}{ \cktsetbasexandyvec \pgfpointxy{30}{30.505} }
\anchor{west}{ \cktsetbasexandyvec \pgfpointxy{-30}{15.2525} }
\anchor{east}{ \cktsetbasexandyvec \pgfpointxy{30}{15.2525} }
\anchor{south west}{ \cktsetbasexandyvec \pgfpointxy{-30}{-6} }
\anchor{south}{ \cktsetbasexandyvec \pgfpointxy{0}{-6} }
\anchor{south east}{ \cktsetbasexandyvec \pgfpointxy{30}{-6} }
\anchor{a}{ \cktsetbasexandyvec \pgfpointxy{-20}{3} \advance\pgf@y by \ycirccenter }
\anchor{b}{
\cktsetbasexandyvec
\pgfpointcurveattime{0.5}%
{\pgfpointxy{-30}{30}}%
{\pgfpointxy{-10}{16}}%
{\pgfpointxy{10}{16}}%
{\pgfpointxy{30}{30}}%
\@tempdima=\baselength
\advance\pgf@y by 6\@tempdima
}
\anchor{c}{ \cktsetbasexandyvec \pgfpointxy{20}{3} \advance\pgf@y by \ycirccenter }
\backgroundpath{
\cktsetbasexandyvec
\cktdraworthreeshape
\cktdraworthreeainversion
\cktdraworthreebinversion
\cktdraworthreecinversion
\cktdrawzinversion
}
}
\pgfdeclareshape{or3nni}{
\inheritsavedanchors[from=nor3iii]
\inheritanchor[from=and2]{center}
\inheritanchor[from=nor3iii]{north west}
\inheritanchor[from=nor3iii]{north}
\inheritanchor[from=nor3iii]{north east}
\inheritanchor[from=or3]{east} % TODO: This is not exact
\inheritanchor[from=or3]{west} % TODO: This is not exact
\inheritanchor[from=or3]{south west}
\inheritanchor[from=or3]{south}
\inheritanchor[from=or3]{south east}
\inheritanchor[from=and2]{tip}
\inheritanchor[from=and2]{z}
\inheritanchor[from=or3]{a}
\inheritanchor[from=or3]{b}
\inheritanchor[from=nor3iii]{c}
\backgroundpath{
\cktsetbasexandyvec
\cktdraworthreeshape
\cktdraworthreecinversion
}
}
\pgfdeclareshape{nor3}{
\inheritsavedanchors[from=nor3iii]
\inheritanchor[from=and2]{center}
\inheritanchor[from=or3]{north west}
\inheritanchor[from=or3]{north}
\inheritanchor[from=or3]{north east}
\inheritanchor[from=or3]{east} % TODO: This is not exact
\inheritanchor[from=or3]{west} % TODO: This is not exact
\inheritanchor[from=nor3iii]{south west}
\inheritanchor[from=nor3iii]{south}
\inheritanchor[from=nor3iii]{south east}
\inheritanchor[from=nand2ii]{tip}
\inheritanchor[from=nand2ii]{z}
\inheritanchor[from=or3]{a}
\inheritanchor[from=or3]{b}
\inheritanchor[from=or3]{c}
\backgroundpath{
\cktsetbasexandyvec
\cktdraworthreeshape
\cktdrawzinversion
}
}

    Status
    API
    Training
    Shop
    Blog
    About

    © 2014 GitHub, Inc.
    Terms
    Privacy
    Security
    Contact


